Toward a Dempster-Shafer theory of concepts

In this paper, we generalize the basic notions and results of Dempster-Shafer theory from predicates to formal concepts. Results include the representation of conceptual belief functions as inner measures of suitable probability functions, and a Dempster-Shafer rule of combination on belief functions on formal concepts.

==> Concepts.tex <==
 

==> Theorem-powerset.tex <==
\redbf{write with the powerset}

In this section, we aim at generalising  Theorem 3.3 from \cite{}, namely \redbf{...}. We proceed as follows ... \redbf{sketch of proof}.


Let $\mathbb{P}=(A,X,I)$ be a finite formal context and ${\mathbb{P}}^+$ be its lattice of concepts. We can assume without loss of generality that $X^{\downarrow}=\varnothing$. We define the polarity $\mathbb{P}'=(A',X',I')$ as follows: 
\begin{itemize}
	\item $A' = X' := L(\mathbb{P})$;
	\item $cId$ if and only if $c\neq d$.
\end{itemize}
\begin{lemma} $\mathbb{P}'^+$ is isomorphic to the 
power set Boolean algebra over the set of all concepts $\mathcal{P}(L(\mathbb{P}))$.
\end{lemma}

Let $c^* \in \mathbb{P}'^+$ be the element $\{c\}$. Notice that the atoms of $\mathbb{P}'^+$ are exactly the elements $\{ c^* \mid c\in \mathbb{P}^+\}$.
  Since $\mathbb{P}'^+$ is a Boolean algebra, we can  define the map $\mu  : \mathbb{P}'^+ \rightarrow [0,1]$ %on the atoms of $\mathbb{A}$ as  
first on the generators of $\mathbb{P}'^+$, by letting
$\mu(c^*)=\mass(c)$ for every $ c\in \mathbb{P}^+$, and  uniquely extend it to a measure on $\mathbb{P}'^+$. 


Let us define the map $h:{\mathbb{P}}^+\hookrightarrow \mathbb{P}'^+$ as follows: 
for every  $c \in \mathbb{P}^+$,
\begin{equation}
h(c)=(\{d\in \mathbb{P}^+ \mid d \leq c\},\{d\in \mathbb{P}^+ \mid d \leq c\}^{\uparrow}).
\end{equation}
Notice that $h(c)=(\{d\in \mathbb{P}^+ \mid d \leq c\},\{d\in \mathbb{P}^+ \mid d \nleq c\})$.

\begin{lemma}
The map $h$ defined above is a meet-preserving embedding.	
\end{lemma}
Let $\iota \ : \ \mathbb{P}'^+ \rightarrow \mathbb{P}^+$ be the right adjoint of $h$.
Let us show that $\bel(c)=\mu_*(c)$ for every $c \in \mathbb{P}^+$. Since $\mathbb{P}'^+$ is an atomic Boolean algebra, every element is equal to the join of the atoms below it.
Furthermore, notice that $d\leq c$ if and only if $d^*\leq h(c)$. Therefore, we have:
%
\begin{align*}
\mu_*(c) & = \mu( \iota(h(c))) =
\mu \left(  
\bigvee \left\{a \in \mathbb{P}'^+ \mid a \leq h(c)
\right\}
\right)
\\ 
& = \mu \left(  
\bigvee \left\{d^* \in \mathbb{P}'^+ \mid d\in \mathbb{P}^+ \; \text{ and } \; d^* \leq h(c)
\right\}
\right)
\tag{because each $a \in \mathbb{P}'^+$ is equal to the join of the atoms below it}
\\
& = \mu \left(  
\bigvee \left\{d^* \in \mathbb{P}'^+ \mid d \leq c
\right\}
\right)
= \sum \{ \mu(d^* ) \mid  d \leq c \}
%\tag{because the $c_*$ form a maximal cover of $\iota (V'(p) )$}
= \sum \{ \mass(d) \mid  d \leq c \}
= \bel_\mass(c).
\end{align*}

Finally, let us show that  $\pl(c)=\mu^*(h(c))$ for every $c \in \mathbb{P}^+$.  Let $U\subseteq{\mathbb{P}}^+$, $c \in \mathbb{P}^+$ and $(d,a) \in A'$. If $(d,a)\in h(c)$, then $(d,a)\in \bigvee_{d\in U}d^*$ if and only if $d\in U$. Furthermore, $(d,a)\in h(c)$ if and only if $a\in\val{c}\cap\val{d}$. Hence, $(d,a)\in h(c)$ implies that $\val{c}\cap\val{d}\neq\emptyset$. We have:

\begin{align}
\bigwedge \left\{ \bigvee_{d\in U}d^* \; \middle| \; U\subseteq{\mathbb{P}}\ \text{ and } \ h(c)\leq \bigvee_{d\in U}d^*\right\}
& = \bigwedge \left\{
\bigvee_{d\in U}d^* \; \middle|  \; \val{d}\cap\val{c}\neq\emptyset \; \text{ implies } \; d\in U \right\}
\notag
\\
& =\bigvee\{d^*\mid \val{d}\cap\val{c}\neq\emptyset\}.
\label{align:proof:th:pl}
\end{align}  
The last equality holds because $\mathbb{A}$ is a Boolean algebra. Hence, we have:
$\bigwedge\{a\in \mathbb{A}\mid c\leq e(a)\}$
\begin{align*}
\mu^*(c) & = \mu(\gamma(h(c)))  
= \mu \left(  \bigwedge\{a\in \mathbb{A} \mid h(c)\leq e(a)\} \right)
\\
& =  \mu \left(\bigwedge
\left\{\bigvee_{d\in U}d^* \; \middle| \; U\subseteq{\mathbb{P}}\ \text{ and }\ h(c)\leq \bigvee_{d\in U}d^*\right\}\right)
\tag{because each $a \in \mathbb{A}$ is equal to the join of the atoms $d^*$ below it}
%\\
%& = \mu \left(\bigwedge\{\bigvee_{d\in U}d^*\mid U\subseteq{\mathbb{P}}\ \&\ h(c)\leq \bigvee_{d\in U}d^*\}\right)
\\
& = \mu \left( \bigvee \{ d^* \mid \val{c} \cap \val{d} \neq \emptyset \} \right)
\tag{see \eqref{align:proof:th:pl}}
\\
& = \Sigma \{ \mu ( d^* ) \mid \val{c} \cap \val{d} \neq \emptyset \} 
\tag{because $\mu$ is additive}
%\tag{because the $c_*$ form a maximal cover of $\gamma (V'(p) )$}
\\
& = \Sigma \{ \mass (d) \mid \val{c} \cap \val{d} \neq \emptyset \} 
 = \pl_\mass (c).
\end{align*}


This concludes the proof of Theorem \ref{th:3.3forlat}.

\begin{theorem}\label{th:3.3forlat}
\redfootnote{\textbf{Reviewer 1.} the construction of $P'$ (for proof of Theorem 3.4; page 5) is needlessly complicated. To have a Boolean algebra of concepts, we can simply having $A' = X' = L(P)$ (i.e. set of all concepts of $P$) and the incidence relation being inequality.
Then the corresponding concept lattice has the set extent equal to power set of $L(P)$.
Much of the rest becomes much simpler, sometimes even trivial, and still equivalent.
I recommend to rework the paper in this manner.}
	For any conceptual DS-structure $\mathbb{D}=(\mathbb{P},\mass)$ there exists a  finite conceptual probability space $\mathbb{X} = (\mathbb{P}', \mathbb{A}, \mu)$, and a meet-preserving embedding $h:{\mathbb{P}}^+\hookrightarrow \mathbb{P}'^+$ such  that $\bel_\mass(c)=\mu_*(h(c))$ and $\pl_\mass(c)=\mu^*(h(c))$.
\end{theorem}


\redfootnote{\textbf{Reviewer 2.} \\
- Section 3.2 seeks to prove Theorem 3.4, which is announced at the beginning and is demonstrated using a series of intermediate results presented throughout this section. In my opinion,  a reorganization of this section would also help to facilitate the reading.\\
- 
%After Theorem 3.4, it is not clear if the definition of this new formal context is given either for a fixed concept "c" or for all the concepts $c\in P^+$.  
I think that the inclusion of examples along the paper would help to understand the new defined structure. }

\bigskip

\redbf{------------------}
